Beyond Accuracy: Statistical Measures and Benchmark for Evaluation of Representation from Self-Supervised Learning

Recently, self-supervised metric learning has raised attention for the potential to learn a generic distance function. It overcomes the limitations of conventional supervised one, e.g., scalability and label biases. Despite progress in this domain, current benchmarks, incorporating a narrow scope of classes, stop the nuanced evaluation of semantic representations. To bridge this gap, we introduce a large-scale benchmark with diversity and granularity of classes, Statistical Metric Learning Benchmark (SMLB) built upon ImageNet-21K and WordNet. SMLB is designed to rigorously evaluate the discriminative discernment and generalizability across more than 14M images, 20K classes, and 16K taxonomic nodes. Alongside, we propose novel evaluation metrics -- `overlap' for separability and `aSTD' for consistency -- to measure distance statistical information, which are efficient and robust to the change of class number. Our benchmark offers a novel perspective of evaluating the quality of representations beyond accuracy. Our findings reveal the limitations of supervised learning and the class bias inherent in SSL models, offering insights into potential areas for future model enhancement.

==> tabs/separability.tex <==

\begin{table}[]
    \centering
    \begin{tabular}{lrrr}
\toprule
{} &  overlap &  mean\_intra &  mean\_inter \\
model &          &             &             \\
\midrule
MSN   &    0.000 &       0.000 &       0.000 \\
iBOT  &    0.619 &       0.237 &       0.076 \\
MMC   &    0.620 &       0.684 &       0.561 \\
DINO  &    0.694 &       0.247 &       0.147 \\
MAE   &    0.751 &       0.426 &       0.243 \\
\bottomrule
\end{tabular}
\caption{Separability for patch features without BN.}
\label{tab:sep_wo}
\vspace{2mm}

\begin{tabular}{lrrr}
\toprule
{} &  overlap &  mean\_intra &  mean\_inter \\
model &          &             &             \\
\midrule
MAE   &    0.550 &       0.171 &       0.038 \\
iBOT  &    0.645 &       0.185 &       0.024 \\
MSN   &    0.691 &       0.114 &      -0.022 \\
DINO  &    0.693 &       0.097 &      -0.030 \\
MMC   &    0.776 &       0.569 &       0.485 \\
\bottomrule
\end{tabular}
\caption{Separability for patch features with BN.}
\label{tab:sep_w}
\vspace{2mm}

\begin{tabular}{lrrr}
\toprule
{} &  overlap &  mean\_intra &  mean\_inter \\
model &          &             &             \\
\midrule
MSN   &    0.000 &       0.000 &       0.000 \\
iBOT  &    0.104 &       0.498 &       0.089 \\
DINO  &    0.112 &       0.490 &       0.107 \\
MMC   &    0.215 &       0.652 &       0.311 \\
MAE   &    0.755 &       0.924 &       0.899 \\
\bottomrule
\end{tabular}
\caption{Separability for CLS features without BN.}
\label{tab:my_label}
\vspace{2mm}

\begin{tabular}{lrrrr}
\toprule
{} &  overlap &  overlap1 &  mean\_intra &  mean\_inter \\
model &          &           &             &             \\
\midrule
DINO  &    0.110 &     0.372 &       0.391 &      -0.008 \\
MAE   &    0.377 &     0.879 &       0.298 &      -0.006 \\
MMC   &    0.137 &     0.488 &       0.447 &      -0.006 \\
MSN   &    0.119 &     0.353 &       0.450 &      -0.008 \\
iBOT  &    0.104 &     0.335 &       0.398 &      -0.008 \\
\bottomrule
\end{tabular}

\caption{Separability for CLS features with BN.}
\label{tab:my_label}
\vspace{2mm}

\end{table}
